OptFlow: Fast Optimization-based Scene Flow Estimation without Supervision

Scene flow estimation is a crucial component in the development of autonomous driving and 3D robotics, providing valuable information for environment perception and navigation. Despite the advantages of learning-based scene flow estimation techniques, their domain specificity and limited generalizability across varied scenarios pose challenges. In contrast, non-learning optimization-based methods, incorporating robust priors or regularization, offer competitive scene flow estimation performance, require no training, and show extensive applicability across datasets, but suffer from lengthy inference times. In this paper, we present OptFlow, a fast optimization-based scene flow estimation method. Without relying on learning or any labeled datasets, OptFlow achieves state-of-the-art performance for scene flow estimation on popular autonomous driving benchmarks. It integrates a local correlation weight matrix for correspondence matching, an adaptive correspondence threshold limit for nearest-neighbor search, and graph prior rigidity constraints, resulting in expedited convergence and improved point correspondence identification. Moreover, we demonstrate how integrating a point cloud registration function within our objective function bolsters accuracy and differentiates between static and dynamic points without relying on external odometry data. Consequently, OptFlow outperforms the baseline graph-prior method by approximately 20% and the Neural Scene Flow Prior method by 5%-7% in accuracy, all while offering the fastest inference time among all non-learning scene flow estimation methods.

==> iccv2023AuthorKit/tables/nsfp_vs_optflow.tex <==
\begin{table*}[t!]
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{@{}lrcccccccccccccccccc@{}}
\toprule
 &\multicolumn{4}{c}{\thead{\textbf{FlyingThings3D}~\cite{ft3d} \\ \small \textit{\#Test: 2,000}}} &\hphantom &\multicolumn{4}{c}{\thead{\textbf{KITTI Scene Flow}~\cite{kitti} \\ \small \textit{\#Test: 50}}} &\hphantom &\multicolumn{4}{c}{\thead{\textbf{Argoverse Scene Flow}~\cite{argoverse} \\ \small \textit{\#Test: 212}}} &\hphantom &\multicolumn{4}{c}{\thead{\textbf{nuScenes Scene Flow}~\cite{nuscenes} \\ \small \textit{\#Test: 310}}} \\
\cmidrule{2-20} 
&\thead{$EPE$ \\ $(m)$} &\thead{$\%_5\uparrow$ \\ $(\%)$} &\thead{$\%_{10}\uparrow$ \\ $(\%)$} &\thead{$\theta_{\epsilon}\downarrow$ \\ $(rad)$} &&\thead{$EPE$ \\ $(m)$} &\thead{$\%_5\uparrow$ \\ $(\%)$} &\thead{$\%_{10}\uparrow$ \\ $(\%)$} &\thead{$\theta_{\epsilon}\downarrow$ \\ $(rad)$} &&\thead{$EPE$ \\ $(m)$} &\thead{$\%_5\uparrow$ \\ $(\%)$} &\thead{$\%_{10}\uparrow$ \\ $(\%)$} &\thead{$\theta_{\epsilon}\downarrow$ \\ $(rad)$} &&\thead{$EPE$ \\ $(m)$} &\thead{$\%_5\uparrow$ \\ $(\%)$} &\thead{$\%_{10}\uparrow$ \\ $(\%)$} &\thead{$\theta_{\epsilon}\downarrow$ \\ $(rad)$} \\ \toprule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\tabitem\textbf{FlowNet3D}~\cite{flownet3d} &0.134 &22.64 &54.17 &0.305     &&0.199 &10.44 &38.89 &0.386     &&0.455 &1.34 &6.12 &0.736       &&0.505 &2.12 &10.81 &0.620 \\
\tabitem\textbf{PointPWC-Net}~\cite{pointpwc} &\textbf{0.121} &{29.09} &\textbf{61.70} &\textbf{0.229}      && {0.142} & {29.91} & {59.83} & {0.239}    && {0.405} & {8.25} & {25.47} & {0.674}    && {0.442} & {7.64} & {22.32} & {0.497} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\arrayrulecolor{black}\bottomrule
\vspace{0.01ex}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\tabitem\textbf{JGF}~\cite{Mittal_2020_CVPR} &\multicolumn{4}{c}{---}   &&0.218 &10.17 &34.38 &0.254     &&0.542 &8.80 &20.28 &0.715        &&0.625 &6.09 &0.139 &0.432 \\
\tabitem\textbf{PointPWC-Net}~\cite{pointpwc} &\multicolumn{4}{c}{---}     &&0.177 &13.29 &42.15 &0.272    &&0.409 &9.79 &29.31 &0.643    &&0.431 &6.87 &22.42 &0.406 \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\arrayrulecolor{black}\bottomrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\tabitem\textbf{Non-rigid ICP}~\cite{amberg} &0.339 &14.05 &35.68 &0.480     &&0.338 &22.06 &43.03 &0.460    &&0.461 &4.27 &13.90 &0.741     &&0.402 &6.99 &21.01 &0.492 \\
\tabitem\textbf{Graph Prior}~\cite{graphprior} &{0.259} &{16.30} & {41.60} & {0.369}     && {0.093} & {64.76} & {82.13} & {0.137}   && {0.257} & {25.26} & {47.50} & {0.467}    && {0.288} & {20.19} & {43.59} & {0.337} \\
\tabitem{\textbf{NSFP}}~\cite{nsfp} &0.234 &19.16 &46.74 &0.341 && 0.050 &81.68 &93.19 &0.133 && \textbf{0.159} &38.43&63.08 &\textbf{0.374} && \textbf{0.175}  &35.18 &63.45&0.279 \\
\tabitem{\textbf{OptFlow (ours)}} & {0.224} & \textbf{31.73} & {57.1}  & {0.340} && {0.052} & \textbf{84.3} & \textbf{93.2} &\textbf{0.130} && {0.20}  &\textbf{43.85} &\textbf{65.5}&{0.39} &&{0.216}&\textbf{40.85}&\textbf{65.97} &\textbf{0.271}\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\arrayrulecolor{black}\bottomrule
\end{tabular}
\end{adjustbox}
\vspace{0.01ex}
\caption{\textbf{Results on 2048 points with no point cloud range limit set.} Comparison with prior work as reported in the NSFP \cite{nsfp}. Top section between shows \textit{off-the-shelf} \textbf{supervised learning methods}; the middle section shows \textbf{self-supervised learning methods}; and the bottom section shows \textbf{non-learning-based methods}. Here $EPE$ denotes the end-point error, $\%_{5}$ denotes strict accuracy,$\%_{10}$ denotes relaxed accuracy and $\theta_{\epsilon}$ denotes angle error.}
\label{tab:main_table_2}
\end{table*}

